Efficient Distance Approximation for Structured High-Dimensional Distributions via Learning

We design efficient distance approximation algorithms for several classes of structured high-dimensional distributions. Specifically, we show algorithms for the following problems: - Given sample access to two Bayesian networks $P_1$ and $P_2$ over known directed acyclic graphs $G_1$ and $G_2$ having $n$ nodes and bounded in-degree, approximate $d_{tv}(P_1,P_2)$ to within additive error $\epsilon$ using $poly(n,\epsilon)$ samples and time - Given sample access to two ferromagnetic Ising models $P_1$ and $P_2$ on $n$ variables with bounded width, approximate $d_{tv}(P_1, P_2)$ to within additive error $\epsilon$ using $poly(n,\epsilon)$ samples and time - Given sample access to two $n$-dimensional Gaussians $P_1$ and $P_2$, approximate $d_{tv}(P_1, P_2)$ to within additive error $\epsilon$ using $poly(n,\epsilon)$ samples and time - Given access to observations from two causal models $P$ and $Q$ on $n$ variables that are defined over known causal graphs, approximate $d_{tv}(P_a, Q_a)$ to within additive error $\epsilon$ using $poly(n,\epsilon)$ samples, where $P_a$ and $Q_a$ are the interventional distributions obtained by the intervention $do(A=a)$ on $P$ and $Q$ respectively for a particular variable $A$. Our results are the first efficient distance approximation algorithms for these well-studied problems. They are derived using a simple and general connection to distribution learning algorithms. The distance approximation algorithms imply new efficient algorithms for {\em tolerant} testing of closeness of the above-mentioned structured high-dimensional distributions.

==> conclusion.tex <==
\section{conclusion}

The main contribution of this paper is to give algorithms to additively approximate the total variation distance beween certain classes of high dimensional distributions. In particular we assume these distribution can be sampled and approximately evaluated on any desired point in its sample space. Often for classes of distributions including bayes nets, causal bayes nets, ising models, and multidimensional Gaussians, approximate evaluations come via learning algorithms for these classes which uses sampling. We relied on this connection to give distance approximation for the above classes of distributions.

==> tester_old.tex <==
\begin{theorem}[\cite{DBLP:conf/colt/CanonneDKS17}]\label{thm:bnlearn}
Given samples from a distribution $P$ on a bayes net of known structure of degree $d$ on $n$ variables each on sample space $\Sigma$ there exists an algorithm that takes $O(|\Sigma|^{d}n(\log n+d)/\epsilon^2)$ samples from $P$ and outputs a distribution $\hat{P}$ on a bayes net with the same structure as that of $P$ such that $\dtv(P,\hat{P})\le \epsilon$ with probability at least 9/10. 
\end{theorem}

We use the following algorithm from~\cite{DBLP:conf/icalp/CanonneR14} for estimating the distance between two high dimensional distributions. We give a proof of their result for completeness. 

\begin{theorem}[\cite{DBLP:conf/icalp/CanonneR14}]\label{thm:dtvest}
Let $P$ and $Q$ be two distributions which we can obtain independent samples from, as well as can evaluate the probability value of any item in the sample space efficiently. Then there is an algorithm that takes $O(1/\epsilon^2)$ samples and $O(1/\epsilon^2)$ evaluations from $P$ and $Q$ each and estimates $\dtv(P,Q)$ up to an additive error $\epsilon$ with probability at least 9/10.
\end{theorem}
\begin{proof}
Let the sample space of $P$ and $Q$ be $\{1,2,\dots,n\}$ without loss of generality.
\begin{align*}
\dtv(P,Q)&={1\over 2}\sum_i |P_i-Q_i|\\
&=\sum_{i:P_i>Q_i} (P_i-Q_i)\\
&=\sum_{i:P_i>Q_i} (1-Q_i/P_i)P_i &&\tag{Since $P_i\neq 0$}\\
&=\sum_{i} 1_{P_i>Q_i}(1-Q_i/P_i)P_i\\
&=\argex{P_i}{1_{P_i>Q_i}(1-Q_i/P_i)} \\ 
\end{align*}
Note that $1_{P_i>Q_i}(1-Q_i/P_i)$ is a number between $[0,1]$. We can estimate the last expectation up to additive error $\epsilon$ with probability at least $(1-\delta)$ by averaging $O({1\over\epsilon^2}\log {1\over \delta})$ samples from Chernoff's bound. We need sampling access to one of the distributions and evaluation access to both the distributions.
\end{proof}

We get a tolerant identity tester for bayes nets by combining Theorems~\ref{thm:bnlearn} and Theorem~\ref{thm:dtvest}.

\begin{theorem}
Given samples from two distributions $P$ and $Q$ on two bayes nets of known structure of degree at most $d$ on a common set $n$ variables each on sample space $\Sigma$, we can test $\dtv(P,Q)\le \epsilon$ versus $>2\epsilon$ using $O(|\Sigma|^{d}n(\log n+d)/\epsilon^2)$ samples with probability at least 2/3.
\end{theorem}

\begin{proof}
First we learn $P$ and $Q$ up to $\dtv$ distance $\epsilon/10$ as $\hat{P}$ and $\hat{Q}$ respectively using Theorem~\ref{thm:bnlearn}. Note that $\hat{P}$ and $\hat{Q}$ are both completely specified bayes nets. For such a bayes net, we first evaluate/sample the root nodes by following its specified distribution. Then we sample/evaluate the nodes which only depend on the root nodes by following appropriate conditional distributions. In this manner we can sample from/evaluate any specified bayes net. We estimate $\dtv(\hat{P},\hat{Q})$ up to additive error $\epsilon/10$ using Theorem~\ref{thm:dtvest}. We decide based on whether the later quantity is $\le 1.3\epsilon$ versus $\ge 1.7 \epsilon$.
\end{proof}
